Accelerating Polynomial Multiplication for Homomorphic Encryption on GPUs

Homomorphic Encryption (HE) enables users to securely outsource both the storage and computation of sensitive data to untrusted servers. Not only does HE offer an attractive solution for security in cloud systems, but lattice-based HE systems are also believed to be resistant to attacks by quantum computers. However, current HE implementations suffer from prohibitively high latency. For lattice-based HE to become viable for real-world systems, it is necessary for the key bottlenecks - particularly polynomial multiplication - to be highly efficient. In this paper, we present a characterization of GPU-based implementations of polynomial multiplication. We begin with a survey of modular reduction techniques and analyze several variants of the widely-used Barrett modular reduction algorithm. We then propose a modular reduction variant optimized for 64-bit integer words on the GPU, obtaining a 1.8x speedup over the existing comparable implementations. Next, we explore the following GPU-specific improvements for polynomial multiplication targeted at optimizing latency and throughput: 1) We present a 2D mixed-radix, multi-block implementation of NTT that results in a 1.85x average speedup over the previous state-of-the-art. 2) We explore shared memory optimizations aimed at reducing redundant memory accesses, further improving speedups by 1.2x. 3) Finally, we fuse the Hadamard product with neighboring stages of the NTT, reducing the twiddle factor memory footprint by 50%. By combining our NTT optimizations, we achieve an overall speedup of 123.13x and 2.37x over the previous state-of-the-art CPU and GPU implementations of NTT kernels, respectively.

==> sections/07_performance_analysis.tex <==
%  ____            __                                           
% |  _ \ ___ _ __ / _| ___  _ __ _ __ ___   __ _ _ __   ___ ___ 
% | |_) / _ \ '__| |_ / _ \| '__| '_ ` _ \ / _` | '_ \ / __/ _ \
% |  __/  __/ |  |  _| (_) | |  | | | | | | (_| | | | | (_|  __/
% |_|   \___|_|  |_|  \___/|_|  |_| |_| |_|\__,_|_| |_|\___\___|

%     _                _           _     
%    / \   _ __   __ _| |_   _ ___(_)___ 
%   / _ \ | '_ \ / _` | | | | / __| / __|
%  / ___ \| | | | (_| | | |_| \__ \ \__ \
% /_/   \_\_| |_|\__,_|_|\__, |___/_|___/
%                        |___/           



% \section{Performance Analysis of Polynomial Multiplication}


% THere is no detailed performance analysis done on GPU in other work.

% \subsection{Modular Multiplication}


% \subsection{Negacyclic Convolution}




% NTT Comparisons:
% \begin{enumerate}
%     \item Naive throughput implementation (Builtin / Barrett Algo 4)
%     \item Single kernel implementation (Builtin / Barrett Algo 4 / RADIX 2 / 4 / 16)
%     \item Multi kernel implementation (Builtin / Barrett Algo 4 / RADIX 2 / 4 / 16)
%     \item Hybrid kernel implementation (Builtin / Barrett Algo 4 / RADIX 2 / 4 / 16)
%     \item Fused NTT
    
% \end{enumerate}


% %mention that $\N=2^{16}$ is default value in HEANN; give the numbers of good primes; mention that it may be possible to define particularly fast NTT's if small powers of 2 are roots of unity; give these counts; discuss 10's of ``good'' primes needed for HE (cite Jung et al or F1?)

% \newpage
% \newpage

% Contributions:
% \begin{enumerate}
%     \item Compare Modular Multiplication algorithms
%     \item Base mod mult (Uses 64 bits)
%     \item 32 Bit implementation that we built
%     \item Implement a faster 32 bit implementation
%     \item Poppelmann's 8 bit modular multiplication SMAS2
%     \item Barett Modular Multiplication (Pre computed value)
%     \item Shoup's Modular Multiplication
%     \item Montgommery Modular Multiplication
%     \item Pre-computed Omega value runtime
%     \item On the fly omega generation
%     \item Mixed omega generation
%     \item $\frac{1}{n}$ scaling: 3 different ways to compute
%     \item Ordering of for loops and loop unrolling in NTT.
%     \item Our entire NTT implentation
% \end{enumerate}

% Novelty:
% \begin{enumerate}
%     \item Different RADIX 2, 4, 16
%     \item Ozerk optimize for latency, we optimize for throughput (Keep the throughput optimized implementation in the paper as well)
%     \item Double butterfly operation (Increase locality)
%     \item 
%     \item GPU optimizations tailored for NTT
%     \item Partitioning techniques (Workload specific)
%     \item New modular multiplication with constant bit width
%     \item MultiGPU scaling for CKKS
% \end{enumerate}

% Motivation:
% \begin{enumerate}
%     \item HE as a whole
%     \item Where NTT fits in
%     \item Problems at hand in NTT
%     \item How it affects HE
%     \item Need for a fast poly mult in HE
%     \item Why it is difficult to implement on GPU
% \end{enumerate}




% \begin{enumerate}
%     \item Benchmarking modular multiplication
%     \item On the fly compute vs Pre-compute of Omega / phi
%     \item NTT Section.
%     \item Subsection: Locality by data rearrangement
%     \item Subsection: Data access patterns, for loop ordering
%     \item Subsection: Loop unrolling
%     \item Data partitioning (Scheduling limbs on streams)
%     \item Speedup on Poly Mult as a whole
% \end{enumerate}

% What percent of entire HE mult workload is Poly Mult or NTT.

% 1 HE Mult = 4 poly mult and 2 HE adds

% Fit HE mult into entire HE.


==> util/word_count.tex <==
% __        __            _    ____                  _   
% \ \      / /__  _ __ __| |  / ___|___  _   _ _ __ | |_ 
%  \ \ /\ / / _ \| '__/ _` | | |   / _ \| | | | '_ \| __|
%   \ V  V / (_) | | | (_| | | |__| (_) | |_| | | | | |_ 
%    \_/\_/ \___/|_|  \__,_|  \____\___/ \__,_|_| |_|\__|


\begin{table}[ht]
	\centering % used for centering table
	\begin{tabular}{l c c} % centered columns (4 columns)
		\hline\hline %inserts double horizontal lines
		\textbf{Section} & \textbf{Word Count} & \textbf{Char Count} \\ [0.5ex] % inserts table
		%heading
		\hline % inserts single horizontal line
		Abstract & \quickwordcount{sections/01_abstract} & \quickcharcount{sections/01_abstract} \\
% 		Version 3 & 94.1\% \\ [1ex]
		\hline %inserts single line
	\end{tabular}
	\caption{Word counts for all sections} % title of Table
	\label{table:word_counts} % is used to refer this table in the text
\end{table}
